3MASSIV: Multilingual, Multimodal and Multi-Aspect dataset of Social Media Short Videos

We present 3MASSIV, a multilingual, multimodal and multi-aspect, expertly-annotated dataset of diverse short videos extracted from short-video social media platform - Moj. 3MASSIV comprises of 50k short videos (20 seconds average duration) and 100K unlabeled videos in 11 different languages and captures popular short video trends like pranks, fails, romance, comedy expressed via unique audio-visual formats like self-shot videos, reaction videos, lip-synching, self-sung songs, etc. 3MASSIV presents an opportunity for multimodal and multilingual semantic understanding on these unique videos by annotating them for concepts, affective states, media types, and audio language. We present a thorough analysis of 3MASSIV and highlight the variety and unique aspects of our dataset compared to other contemporary popular datasets with strong baselines. We also show how the social media content in 3MASSIV is dynamic and temporal in nature, which can be used for semantic understanding tasks and cross-lingual analysis.

==> figures/video-type.tex <==
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.3\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figures/split-screen-1.png}
         \caption{Split Screen}
         \label{fig:splitscreen}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figures/animation-1.png}
         \caption{Animation}
         \label{fig:animation}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figures/text-overlay-1.png}
         \caption{Text Overlay}
         \label{fig:reaction}
     \end{subfigure}
      \caption{\textbf{Unique video types in \datasetname:} (a) Split-screen videos tend to have multiple embedded visuals running simultaneously on the same screen; (b) Animation clips are digital-borne videos; (c) Videos with text overlay words on pre-recorded videos. Text can be either transcriptive, referential or descriptive in nature.}
     \label{fig:video_types}
\end{figure}


==> sections/concept.tex <==
\section{What is \concept?}
\label{sec:concept}

\concept is a higher-order, holistic and abstract idea that goes beyond recognizing the \visualdim like objects, scene or affective states. In Figure 1, the presence of objects (chair, mic, lights, human), emotional state (happiness, excitement), scene (stage) etc. can be detected by using a state-of-the-art deep learning models which can process the pixels of the videos. However, the \concept (\textit{comedy} in this example) lies beyond the pixels and can not be ascertained by a mere presence or absence of objects. While, for some of the \concepts like \textit{sports} or \textit{food}, comparatively higher correlation exists between \visualdim and \concept but presence of these \visualdim can not guarantee \concept recognition. Recognizing the \concept requires modelling the interplay between \visualdim making it an extremely difficult and challenging problem. Similar observations can be made about a romantic scene, travel video, health video or pet video where the scene (garden, road, kitchen, home) or objects (bike, house, food, humans) play a part but can not determine the core \concept. \vikram{Let us talk about Figure 1 to Figure 4 here in detail. Explain how \concept is important in these cases}

\section{Inter-agent Relationships}
\label{sec:relations}
\vikram{I guess we can write few words about this aspect as well. Not sure about the best place to mention these}
\section{Affective States}
\label{sec:relations}
\vikram{I guess we can write few words about this aspect as well. Not sure about the best place to mention these}


==> sections/experiments.tex <==
\section{Current and Future Tasks}
\label{sec:tasks}
\begin{itemize}
\item Video Classification : Multimodal - Audio + Video + Face + NLU (natural language understanding) layer
\item Emotion Understanding
\item Culture Understanding : Zero shot and transfer learning
\item Language Identification from audio channel
\item Behaviour and relationship modelling
\item Multitask learning - predict audio, video types and language also as auxiliary task.
\end{itemize}


\section{Experiments}
\label{sec:experiments}
\begin{itemize}
\item 
\end{itemize}

\section{Data and User Privacy}
\label{sec:data_privacy}
The videos were collected from publicly available Moj platform. An informed consent of the users was taken for public usage of these videos and Moj holds the rights to these videos. The User Ids and exact date of publication has been masked off to protect privacy. The dataset would only be available for research purposes. 
\begin{table*}[t]
\centering
\begin{tabular}{llcccc}
\toprule
Modality & Backbone & Fusion & Top-1 Accuracy & Top-3 Accuracy & Top-5 Accuracy \\
\midrule
Video & Resnext3D(50) & - & 49.7 & 67.9 & 75.3 \\
Video & Resnext3D(100) Features & - & 49.7 & 67.7 & 75.3 \\
\midrule
Audio & VGG & - & - & - & - \\
Audio & CLSRIL-23 & - & - & - & - \\
\midrule
Video, Audio & Resnext3D(50) + VGG  & Late & 54.5 & 75.6 & 83.4 \\
Video, Audio & Resnext3D(50) + CLSRIL-23 & Late & 54.7 & 75.1 & 82.9 \\
Video, Audio & Resnext3D(50) + VGG + CLSRIL-23 & Late & \textbf{56.1} & \textbf{77.0} & \textbf{84.3} \\
\bottomrule
\end{tabular}
\caption{\textbf{\concept Classification}}
\label{tab: topic_classification}
\end{table*}




==> sections/extra.tex <==
However, the content uploaded on social media platforms as well in practical situations are more nuanced with even non-human actors like pets, food items, scenery, videos, gadgets etc. playing the key role. Even with human actors, different concepts or themes like husband-wife comedy, couple romance, pranks,  etc exist but do not fall under the purview of typical human action understanding as these require a deeper understanding of facial/body emotions and interplay between the actors. In this work, we contribute a novel culturally (language/geography-zones) diverse, truly-multimodal (since audio plays an important role) and multilingual (10 Indic languages), video dataset \datasetname with diverse semantic content focussed on human, animals and even non-animate actors.

\subsection{Data Uniqueness}
\label{sec:data_uniqeness}

We analyze and annotated the videos of few days to identify the themes that capture the majority of the content. Using those themes, we select 26 classes for final dataset.


\begin{itemize}
    \item \textbf{Diverse Actors:} Our dataset tries to capture the themes and trends expressed on short video platforms. Not only limited to human action understanding (sports, dance, health and fitness) but also to animals (animals, pets) and non-animate (nature, food) actors. While human action categories can be solved by focusing on motion of the human actors, other categories require understanding of the overall context, scene, objects etc.
    \item \textbf{Affective States:} We also annotate the emotions projected by the creators of the video which can be used for studying affective states.
    \item \textbf{Diverse video types:} Our dataset contains variety of audio and video formats which are unique to social media videos, especially short video platforms. Dataset has self-shot videos, movie/tv-serial clippings, slideshows, animations, split screen videos etc. Some videos are also overlaid with special effects and texts. 
    \item \textbf{Diverse audio types:} The audio formats comprise of recorded and self-sung songs, background instrumental music spoken monologues and dialogues etc. Some videos have just background noise.
    \item \textbf{Multimodal:} Our taxonomy is rich for modelling interplay between audio and visual modality. For ex. some categories like music, comedy, romance, dance have strong audio signals while categories like food, nature might not have audio as a relevant channel. Our audio contains songs, music as well as spoken text. NLU can also be helpful to understand the spoken text and classify videos using the text ex. astrology. For categories like celeb, even modelling the identity could be useful. 
    \item  \textbf{Multilingual:} Our dataset has videos from 10 Indic languages allowing for integrating natural language understanding for video classification. We can show empirically or analytically that language plays a part for our datasets. For ex. categories like astrology, gadgets, automobiles, technology can benefit by understanding what is being spoken.
    \item \textbf{Culturally Diverse:} Dataset is sourced from users belonging to X Indian states and speaking 10 Indian languages. This can provide an opportunity to study the cultural and linguistic bias of users on our platform.
    \item \textbf{Behaviour and relationship modelling:} Our dataset has topics which are more fine and require deeper understanding like comedy, romance. Comedy and Romance have subcategories like pranks, accidents, kids comedy, adult comedy etc. presenting an opportunity to perform human behaviour modelling. 
    \item \textbf{Human Annotation} Each video has been annotated by 3 human annotators who were native to the language of the audio.
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/language_distribution.pdf}
    \caption{Number of samples for the languages in 50K videos}
    \label{fig:lang_dist}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/topic_distribution.pdf}
    \caption{Number of samples for the topics in 50K videos}
    \label{fig:lang_dist}
\end{figure}

==> sections/intro-vik.tex <==
\section{Introduction-2}
\label{sec:intro2}

Understanding the \textit{semantic meaning} of videos has been a long standing and well-researched problem but still continues to garner a lot of attention from the computer vision research community as well as industry. Multiple datasets and challenges are being introduced every year to further advance the field of semantic understanding to address real-life use-cases and applications like augmented reality, content moderation, content recommendation, self-driving cars etc. What makes the problem exciting and extremely challenging is formulating the \textit{meaning} of this \textit{semantic meaning} itself because of the spatio-temporal richness of video content. A video expresses too many things at the same time. For example, let us consider video of a person enacting a comedy scene on a stage in Figure~\ref{fig:standup-comedy}. This video can be understood from multiple semantic dimensions.~\textit{Human action:} It represents a person doing human actions like laughing, walking, speaking etc. \textit{Affective state:} The comedian displays different emotions like happiness/excitement during the act. \textit{Scene:} The act might be happening inside a small auditorium. \textit{Objects:} Video comprises of a human, mic, lights, water bottle and a stool. \textit{Audio:} Audio may have background noise, laughs/claps etc. and corresponding transcriptions may have words representing a joke. 


\noindent\textbf{Concept:} However, these dimensions can be coined as \visualdim as they represent artifacts which are physically present in the video and can be detected using state-of-the-art computer vision algorithms. Detecting these~\textit{visual dimensions} mimics \textit{how humans see this video} but it does not capture \textit{how humans will catalogue and summarize this video? What is the core \concept of this video?}  Typically, humans understand videos by creating an abstract and holistic representation rather than remembering the presence of artifacts. In this work, we model this challenging research question in the realm of social media videos - \textit{How do social media users conceptualize videos? What could be the possible vocabulary of these videos?}

\noindent\textbf{Use Cases:} This is an important research direction for developing more social and humane video understanding models and has tremendous potential for improving the understanding of both the users and videos, particularly in the context of social media. In our previous example, the \concept of the video can be \textit{comedy} which allows us to infer much more about the users' interest and videos' content than simply knowing the presence of mic, lights etc. Using \concept taxonomy, we can explicitly model the likes and dislikes of users in human understandable format creating more transparent models. \concept understanding can help us in understanding the creation, consumption and popularity dynamics of the social media videos and can be instrumental in moderating the content and providing fulfilling user experience. It can also help advertisers and content creators in understanding the kind of videos people like. \visualdim can surely act as a helpful prior for \concept understanding but they do not represent the \concept itself and it would be interesting to see how far \concept understanding can be done using \visualdim. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/standup-comedy.png}
%     \caption{Standup comedy scene}
%     \label{fig:standup-comedy}
% \end{figure}

\noindent\textbf{Image/Text Datasets:} Similar to our work, Intentonomy~\cite{jia2021intentonomy} contribute a dataset of 14K images posted on social media with the annotations representing the 28 human perceived \textit{intent} types supported by systematic social psychological taxonomy~\cite{talevich2017toward} behind these images. They study the extent to which visual information present in the images can facilitate human intent understanding. In this case also, \visualdim do not have a one-to-one mapping with intent. For example,  image of a waterfall and person doing yoga might both represent \textit{peace} as the intent. Similarly, intent and motivation understanding from images/text has been studied by ~\cite{pirsiavash2014inferring, joo2014visual, joo2015automated, huang2016inferring,thomas2019predicting,Vondrick_2016_CVPR,zhang2018equal,wang2019persuasion}.
Focussing on social media,~\cite{kruk2019integrating, souza2015dawn, bakhshi2015we, lee2015people, lai2019motivations} perform similar studies on the motivations on social media images posts.

\noindent\textbf{Video Datasets:}~\cite{siddiquie2015exploiting} focused on videos from RAC dataset on identifying if videos is politically motivated. Similar study has also been performed in the domain of advertisement understanding.~\cite{ye2019interpreting, hussain2017automatic}\vikram{both papers talk about the same dataset and are from same authors, so we need to clear out the difference} present a dataset of 64,832 image ads and 3,477 video ads annotated with 38 topics, 30 sentiments and user actions with explanations which are not audio-visual in nature. The topics (cars, automobiles, education, smoking etc.) are similar in spirit to our \concept taxonomy but they mainly focus on the advertisement videos and the dataset is comparatively smaller than our dataset. The \concept taxonomy provided by HVU dataset~\cite{diba2019holistic} consists of 291 machine generated concepts extracted using Google Vision API\footnote{cloud.google.com/vision} and Sensifai Video Tagging API\footnote{https://sensifai.com/}\footnote{https://demo.sensifai.com/}.\vikram{This concept taxonomy seems relevant to us. We need to compare with them.}

From these datasets, we realize that while \concept or high-level intent/motivations has been studied, understanding them in the videos has been severely limited, probably due to absence of large scale datasets. To fill this gap, we contribute a novel dataset - AVATAR.

\noindent\textbf{AVATAR:} We focus ourselves towards \concept understanding in social media videos posted on short-video application Moj by ShareChat. These videos are created by both professional and amateur creators from over 15 languages. \vikram{We can talk more about the format of Moj here}. Creating a \concept taxonomy which represents popular videos posted and consumed on social media was a challenging task. We began with the objective of using popular tags as \concepts but realized that tags did not represent the \concepts as tags were generally noisy. Moreover, a large number of videos did not have tags associated with them \vikram{We can write it in a better way to show why tags can not be used or were not used. We can quantify how many videos did not have tags to establish this fact.} Thus, we adopted a rigorous bottom-up approach for designing a taxonomy of important and popular \concepts on social media. We used social media interaction (views/likes/shares) as a measure for mining 100 million popular videos over a period of 6 months across 11 languages. Our \concept taxonomy is inspired by human interest expressed on the social media videos.\vikram{We can reiterate it further to showcase the uniqueness of taxonomy creation}  We then analyzed these videos using an expert annotation team and built a novel and comprehensive taxonomy of \concepts for representing every popular video with one \concept category. Due to the subjective nature of \concepts originating from the differences in human perceptions of videos, we noted that obtaining high agreement was non-trivial. Moreover, some videos can even represent more than one \concept. We also noticed hierarchy in the taxonomy and respected it with 2 levels. For ex. \textit{automobiles} have both \textit{car} and \textit{bikes}. Similary, animals have \textit{aquatic}, \textit{pets}, \textit{wild} etc. The taxonomy grew to more than 600 categories and was pruned to X \concepts which had sufficient number of samples. Our videos contain variety of trendy and viral \concepts like comedy, romance, philanthropy, devotion, patriotism etc. which are famous among the social media users. 

\noindent\textbf{Audio Language:} For modelling the natural language dimension, we also annotated the language of the audio. The videos are coming from 11 different languages presenting opportunities for multilingual analysis.

\noindent\textbf{Affective States:} We also wanted to understand the projected emotions in these videos and annotated them with \affectivestate. Instead of modelling evoked emotions which are highly subjective, we selected projected emotions where the idea is to annotated the possible emotion the content creator was trying to express. This can be useful in understanding the emotional well-being of the users and platform and can be instrumental in detecting signs of depression, bullying etc.\vikram{We can cite some papers which support these claims.}

\noindent\textbf{Media Types:} Owing to their origin in social media, we also noticed the diversity of video formats comprising of memes, slide-shows, animations, split-screens, self-shot, movie/TV-serial clips etc. which are very popular on social media. Overlaid text and graphics further make these videos unique and interesting. The audio types are also very unique with recorded/self-sung songs, dialogues, monologues, instrumentals etc. These unique \audiotype and \videotype provide an opportunity for modelling these novel media types which have never been attempted before.  

\noindent\textbf{Viewpoints:} Majority of the videos are captured using hand-held cameras and contain selfie-views, third-person, egocentric etc. views.

\noindent\textbf{Relation Modelling:} We also provide finer annotations for comedy and romance with categories like pranks, fails, humour, philanthropy, one-sided-love, heartbreak etc for modelling deeper human expressions and relationships. 

\noindent\textbf{User Modelling:} Unlike most of the datasets, we also provide masked user ids which can be helpful in learning the user profiles as well.


\noindent\textbf{Timestamps:} Unlike most of the datasets, we also provide timestamps of these videos which can be helpful in modelling temporal dynamics.~\cite{kim2010modeling},~\cite{nguyen2016open} attempted similar studies earlier.

To the best of our knowledge, our dataset - \datasetname is the first human-annotated dataset which captures and annotates these unique \concepts, \affectivestate, \languagetype, \videotype and \audiotype across 11 languages presenting a unique opportunity for modelling higher level \concepts across challenging media types and multilingual settings. We also present baseline results to empirically establish the uniqueness of our dataset.  

In summary our contributions are:
\begin{itemize}
    \item A novel human-annotated \datasetname dataset of 50K (X hours of data) social media videos annotated with a hierarchical taxonomy of X \concept
    \item Annotated \languagetype for modelling multilingual properties in social media posts
    \item \affectivestate annotations for performing emotion analysis over social media videos
    \item Novel \audiotype and \videotype common in social media video presenting new challenges in video understanding
    \item Fine-grained annotations for modelling human relationships and interactions
    \item User and temporal modelling opportunities
\end{itemize}
 
% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{figures/prank1.png}
%     \caption{Prank Scene}
%     \label{fig:prank}
% \end{figure*}
% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{figures/fail1.png}
%     \caption{Fail Scene}
%     \label{fig:fail}
% \end{figure*}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{figures/philanthropy.png}
%     \caption{Philanthropy Scene}
%     \label{fig:kindness}
% \end{figure*}


% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{figures/comedy-strip.png}
%     \caption{Comedy Scene}
%     \label{fig:comedy}
% \end{figure*}



% \begin{figure*}
%      \centering
%      \begin{subfigure}[b]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/split-screen.jpg}
%          \caption{Split Screen}
%          \label{fig:splitscreen}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/animation.jpg}
%          \caption{Animation}
%          \label{fig:animation}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/text_overlay.jpg}
%          \caption{Text and Graphics overlay}
%          \label{fig:reaction}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/text_overlay.jpg}
%          \caption{Text and Graphics overlay}
%          \label{fig:reaction}
%      \end{subfigure}
%         \caption{Video Types}
%         \label{fig:video_types}
% \end{figure*}


% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/comedy_2.png}
%     \caption{Group comedy scene}
%     \label{fig:group-comedy}
% \end{figure}



==> tables/annotator-agreement.tex <==
% \begin{table}[t]
% \centering
% \resizebox{.7\columnwidth}{!}
% {
% \begin{tabular}{ lc} 
% \toprule[1.5pt]
% \textbf{Aspect} & \textbf{Krippendorff's Alpha}\\
% \midrule
%  Concept & 0.77 \\
%  Audio Type  & 0.59 \\
%  Video Type  & 0.62 \\
%  Affective States & 0.40 \\
% \bottomrule[1.5pt]
% \end{tabular}
% }
% \caption{Inter-annotator agreement metrics for \datasetname dataset}
% \label{table:annotation_metrics}
% \end{table}

\begin{table}[t]
\centering
\resizebox{.8\columnwidth}{!}
{
\begin{tabular}{ccccc} 
\toprule
\textbf{Concept} & \textbf{AudioType} & \textbf{VideoType} & \textbf{Affective States}\\
\midrule
0.77 & 0.59 & 0.62 & 0.40 \\
\bottomrule
\end{tabular}
}
\caption{Krippendorff's Alpha for measuring inter-annotator agreement for \datasetname dataset}
\label{table:annotation_metrics}
\end{table}

==> tables/competetitor_datasets_backup.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{threeparttable}
    \begin{tabular}{crcccccccc}
    \toprule[1.5pt]
	&Datasets&	Size& 	Source&	Labels&	Audio Types&	Video Types&	Affective&	Focus & Lang.\\
	\midrule
	\multirow{1}{*}{\rotatebox{0}{Image}} & Intentonomy~\cite{jia2021intentonomy} &	14k & Flickr &	\cellcolor{green!25} HA	&\cellcolor{red!25}-&	\cellcolor{red!25}-& \cellcolor{red!25}NA &	Understanding Intent of Social Media Posts & \cellcolor{red!25} - \\
	%& Flickr30k & 30k &	Flickr & \cellcolor{green!25}HA &	\cellcolor{red!25}-& \cellcolor{red!25} - &	\cellcolor{red!25}NA &	Sentence-Based Image Captioning & \cellcolor{red!25} -\\
	
	\midrule
	
	\multirow{12}{*}{\rotatebox{0}{Video}}&YouTube-8M~\cite{abu2016youtube} &	8M&	YouTube&\cellcolor{red!25} 	MG&\cellcolor{red!25}NA&	 \cellcolor{red!25}NA&	\cellcolor{red!25}NA&	Video Topic Classification&\cellcolor{red!25}NA\\
	& HVU~\cite{diba2019holistic} &	500k &	YT8M, Kinetics, HACS	&\cellcolor{red!25} MG	&\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	Actions, Objects, Concepts, Events, Attributes, Scenes&\cellcolor{red!25} NA\\
	& Epic-Kitchens~\cite{Damen2021PAMI} &	39594 &	Enacted by actors	&\cellcolor{green!25} HA	&\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	Actions in Kitchen &\cellcolor{green!25} Yes\\
	&	MV-58K~\cite{nguyen2016open} & 260k & Vine & \cellcolor{red!25} MG & \cellcolor{red!25}NA &	\cellcolor{red!25}NA	&\cellcolor{red!25}NA	&Activity, Objects, Platform Specific Classes&\cellcolor{red!25} NA\\
	& SOA~\cite{ray2018scenes} & 562k & Facebook & \cellcolor{green!25} HA & \cellcolor{red!25}NA &	\cellcolor{red!25}NA	&\cellcolor{red!25}NA	&Scenes, Objects, Actions &\cellcolor{red!25} NA\\
    &	Kinetics~\cite{kay2017kinetics} &	300k&	YouTube&\cellcolor{green!25} 	HA&	\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	HAR (400/600/700 classes)&\cellcolor{red!25} NA\\
    &	MomentsInTime~\cite{monfort2019moments} &	1M&	10 sources &\cellcolor{green!25} 	HA&	\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	339 action classes &\cellcolor{red!25} NA\\
    &	ActivityNet~\cite{yu2019activitynet} &	27801 &	Web &\cellcolor{green!25} 	HA&	\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	HAR (203 classes) &\cellcolor{red!25} NA\\
    & HACS~\cite{zhao2019hacs} &	1.5M&	YouTube&\cellcolor{green!25} 	HA&	\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	HAR (200 classes)&\cellcolor{red!25} NA\\
	& Something-Something~\cite{goyal2017something} & 100k &	Enacted by crowd workers &\cellcolor{green!25} HA &	\cellcolor{red!25}NA &	\cellcolor{red!25}NA	& \cellcolor{red!25}NA	& HAR (174 classes) & \cellcolor{red!25} NA\\
	&Charades~\cite{zhou2018temporal} &	9848&	Actors&\cellcolor{green!25} 	HA&	\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	HAR + Object Classification (157 classes)&\cellcolor{red!25}NA\\
	
	& Sports-1M~\cite{karpathy2014large} &	1M&	YouTube&\cellcolor{red!25} 	MG&	\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	Sports Activity Classification (487 Classes)&\cellcolor{red!25}NA\\
	\midrule
	\multirow{2}{*}{\rotatebox{0}{Affects (videos)}}&EEV~\cite{sun2020eev} & 23k & Online Videos &\cellcolor{red!25} MG &	\cellcolor{red!25}NA & 	\cellcolor{red!25}NA&	\cellcolor{green!25}Yes&	Evoked EC (15 classes)&\cellcolor{red!25}NA\\
	&	CMU-MOSEI~\cite{zadeh2018multimodal} &23K&		YouTube&\cellcolor{green!25} 	HA&\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	\cellcolor{green!25}Yes&	Perceived EC (6 classes)&\cellcolor{red!25} NA\\
	%& SVD~\cite{jiang2019svd} & 500k & TikTok & \cellcolor{green!25} HA &	\cellcolor{red!25} - &	\cellcolor{red!25}NA&	\cellcolor{red!25}NA&	Near Duplicate Video Retrieval &\cellcolor{red!25}NA\\
	\midrule
	
	
	\multirow{2}{*}{}&\multirow{2}{*}{\textbf{Ours}} &	\multirow{2}{*}{50k(+100k)} & \multirow{2}{*}{Social Media Platform}	&	\cellcolor{green!25}&\cellcolor{green!25}Annotated for&\cellcolor{green!25} Annotated for&	\cellcolor{green!25}&\multirow{2}{*}{Concept, Affective States, Media Type, Language}&\cellcolor{green!25}Annotated for \\	
	
    &&&&  \cellcolor{green!25}\raisebox{2.7ex}[2.7ex]{\multirow{2}{*}{HA}} &\cellcolor{green!25}7 classes&\cellcolor{green!25}8 classes&\cellcolor{green!25}\raisebox{2.7ex}[2.7ex]{\multirow{2}{*}{Yes}}&&\cellcolor{green!25}11 languages \\	
    
    	
    %&&&&  \cellcolor{green!25}\raisebox{2.7ex}[2.7ex]{\multirow{2}{*}{HA}} &\cellcolor{green!25}\raisebox{2.7ex}[2.7ex]{\multirow{2}{*}{7 classes}}&\cellcolor{green!25}\raisebox{2.7ex}[2.7ex]{\multirow{2}{*}{8 classes}}&\cellcolor{green!25}\raisebox{2.7ex}[2.7ex]{\multirow{2}{*}{Yes}}&&\cellcolor{green!25}11 languages \\	
    
	\bottomrule[1.5pt]
    \end{tabular}
    \end{threeparttable}
    }
    \begin{tablenotes}\footnotesize
    \item $^\dagger$ NA, MG, HA indicate ``not annotated'', ``machine generated'', and ``human annotated'', respectively.
    \end{tablenotes}
    
    \caption{Comparison of \datasetname with related image and video datasets. Our dataset has exhaustive and expertly annotated annotations for concepts, audio/video types, affective states and audio language.}
    \label{tab:datasets}
\end{table*}


==> tables/emotion-classification.tex <==
\begin{table}[t]
    \centering
    \resizebox{.8\columnwidth}{!}{
    \begin{tabular}{rcccc}
     \toprule
        Method & Modality & Top-1($\%$)& Top-$3$($\%$) & F1\\
    \midrule
    Kosti et al.~\cite{kosti2017emotic} & visual & $35.08$ & $81.92$ & - \\
    % Tsai et al. \cite{tsai2019multimodal}& audio & - & - & - \\
    % Tsai et al. \cite{tsai2019multimodal}& visual & - & - & - \\
    Tsai et al. \cite{tsai2019multimodal}& audio-visual & $38.05$ & $83.90$ & - \\
     \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Baseline Experiments for Affective State Classification: }We present results for two SOTA affective state classification when evaluated on \datasetname.}
    \label{tab:emotion_classification}
\end{table}

==> tables/topic-ablation.tex <==
\begin{table}[t]
\scriptsize
\centering
%\resizebox{0.8\textwidth}{!}{
\begin{tabular}{llcccc}
\toprule
Modality & Backbone & Top-1 & Top-3 & Top-5 \\
\midrule
Video, Audio & R3D-50 + VGG + CLSRIL23 & \textbf{60.1} & \textbf{81.6} & \textbf{88.5} \\
Video, Audio & R3D-50 + VGG + CLSRIL23 + Creator & \textbf{62.2} & \textbf{83.1} & \textbf{89.4} \\
\bottomrule
\end{tabular}
%}
\caption{Early Fusion}
\label{tab:topic_classification_ablation}
\end{table}

\begin{table}[t]
\scriptsize
\centering
%\resizebox{0.8\textwidth}{!}{
\begin{tabular}{llcccc}
\toprule
Modality & Backbone & Top-1 & Top-3 & Top-5 \\
\midrule
Video & R3D-50 (Layer\_fc\_onwards) & \textbf{53.5} & \textbf{74.5} & \textbf{83.7} \\
Video & R3D-50 (Layer1\_onwards) & \textbf{53.6} & \textbf{74.6} & \textbf{83.5} \\
Video & R3D-50 (Layer4\_onwards)  & \textbf{53.7} & \textbf{74.9} & \textbf{83.2} \\
Video & R3D-101 (Layer4\_onwards)  & \textbf{52.9} & \textbf{74.8} & \textbf{83.5} \\
Video & R3D-101 (Layer1\_onwards)  & \textbf{53.4} & \textbf{74.5} & \textbf{83.7} \\
Video & R2p1D-50 (Layer4\_onwards)  & \textbf{55.0} & \textbf{76.5} & \textbf{84.8} \\
Video & R2p1D-50 (Layer1\_onwards)  & \textbf{55.4} & \textbf{76.3} & \textbf{84.8} \\


\bottomrule
\end{tabular}
%}
\caption{Early Fusion}
\label{tab:topic_classification_fine_tuning}
\end{table}


==> tables/topic-classification.tex <==
\begin{table}[t]
\scriptsize
\centering
%\resizebox{0.8\textwidth}{!}{
\begin{tabular}{llcccc}
\toprule
Modality & Backbone & Top-1 & Top-3 & Top-5 \\
\midrule
Video & R(2+1)D-50 & 50.6 & 72.3 & 81.4 \\
Video & R3D-50 & 52.7 & 74.5 & 83.6 \\
Video & R3D-100 & 52.6 & 74.1 & 83.3 \\
\midrule
Audio & VGG & 31.6 & 50.5 & 60.9 \\
Audio & CLSRIL23 & 31.2 & 50.1 & 60.6 \\
\midrule
Video, Audio & R3D-50 + VGG & 54.9 & 74.9 & 82.4 \\
Video, Audio & R3D-50 + CLSRIL23 & 54.9 & 75.4 & 82.9 \\
Video, Audio & R3D-50 + VGG + CLSRIL23 & \textbf{56.5} & \textbf{76.5} & \textbf{83.8} \\
\bottomrule
\end{tabular}
%}
\caption{Baseline experiments for concept recognition using different modalities and combinations on \datasetname.}
\label{tab:topic_classification}
\end{table}

